Phase resonance nonlinear modes of mechanical systems

The resonances of forced dynamical systems occur when either the amplitude of the frequency response undergoes a local maximum (amplitude resonance) or phase lag quadrature takes places (phase resonance). This study focuses on the phase resonance of nonlinear mechanical systems subjected to single-point, single-harmonic excitation. In this context, the main contribution of this paper is to develop a computational framework which can predict the mode shapes and oscillation frequencies at phase resonance. The resulting nonlinear modes are termed phase resonance nonlinear modes (PRNMs). A key property of PRNMs is that, besides primary resonances, they can accurately characterize superharmonic, subharmonic and ultra-subharmonic resonances for which, as shall be shown in this paper, phase lags at resonance may be different from pi/2. The proposed developments are demonstrated using one- and two-degree-of-freedom systems featuring a cubic nonlinearity.

==> Notes.tex <==
%%% Recueil de notes pour les modifications plus tard,

- Refaire les figures subplot, elles n'ont pas la même taille exactement,

- Revérifier le phasage exact des séries temporelles de la superH 2

- Préciser au début que pour chaque harmonique, le graphe amplitude/fréquence et Phase/fréquence pour l'harmonique considérée sont présentés, afin d'éviter les doublons
